CryoBench: Diverse and challenging datasets for the heterogeneity problem in cryo-EM

Cryo-electron microscopy (cryo-EM) is a powerful technique for determining high-resolution 3D biomolecular structures from imaging data. Its unique ability to capture structural variability has spurred the development of heterogeneous reconstruction algorithms that can infer distributions of 3D structures from noisy, unlabeled imaging data. Despite the growing number of advanced methods, progress in the field is hindered by the lack of standardized benchmarks with ground truth information and reliable validation metrics. Here, we introduce CryoBench, a suite of datasets, metrics, and benchmarks for heterogeneous reconstruction in cryo-EM. CryoBench includes five datasets representing different sources of heterogeneity and degrees of difficulty. These include conformational heterogeneity generated from designed motions of antibody complexes or sampled from a molecular dynamics simulation, as well as compositional heterogeneity from mixtures of ribosome assembly states or 100 common complexes present in cells. We then analyze state-of-the-art heterogeneous reconstruction tools, including neural and non-neural methods, assess their sensitivity to noise, and propose new metrics for quantitative evaluation. We hope that CryoBench will be a foundational resource for accelerating algorithmic development and evaluation in the cryo-EM and machine learning communities. Project page: https://cryobench.cs.princeton.edu.

==> Figures/noise_temp.tex <==
\begin{figure}[h]
  \centering
  \begin{minipage}[h]{0.45\textwidth}
    % \centering
    \includegraphics[width=\textwidth]{Figures/pngs/fig3_noise.pdf}
    \caption{\textbf{IgG-1D Noise.}} (a) AUC of Per-Conformation-FSC for each method at SNR levels of 0.01, 0.005, 0.001, respectively. cryo-EM images at different noise levels are provided. (b) UMAP plots colored by G.T dihedral conformations of RECOVAR and DRGN-AI at different noise levels. Higher noise demonstrates thicker representations.
    \label{fig:fig7_noise}
  \end{minipage}\hfill
  \begin{minipage}[h]{0.45\textwidth}
    \centering
    \resizebox{\textwidth}{!}{ % Resize the table to fit the width of the minipage
    \begin{tabular}[H]{c|c|c}
        % \centering
        \toprule
        \textbf{Method} &
        \textbf{Ribosembly} & \textbf{Tomotwin-100} \\
       % & k= & k=5\%  \\
        \midrule
        CryoDRGN &  \underline{78.84 (0.14)} & \textbf{96.78 (0.13)}\\
        
        DrgnAI-fixed & 76.62 (0.16) & \underline{85.55 (0.08)}  \\
        
        Opus-DSD & 72.53 (0.46) & 50.30 (0.17) \\
        
        3DVA & 72.05 (0.15) & 11.80 (0.05)  \\
        
        RECOVAR & \textbf{78.89 (0.06)}& 39.89 (0.19)\\
        \midrule

        CryoDRGN2 &  53.37 (0.12)& \textbf{15.01 (0.07)}\\
        DrgnAI-abinit & \textbf{66.27 (0.14)}& 11.13 (0.14)\\
        \bottomrule
      \end{tabular}
      }
    \captionof{table}{\textbf{Ribosembly and Tomotwin-100 percentage of correct structural clustering.} Percentage of matching neighbors (Eq. \ref{eq:neigh_sim}) with $k$ equal to the number of ground truth images per structure. The mean from five independent subsets is presented, and standard deviation of the mean is shown in parenthesis.}
    \label{tab:tab2_cluster}
  \end{minipage}
\end{figure}





% \begin{figure}[h]
%   \centering
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/pngs/Fig7_noise.pdf}
%     \caption{IgG-1D Noise.} (a) AUC of Per-Conformation-FSC for each method at SNR levels of 0.01, 0.005, 0.001, respectively. cryo-EM images at different noise levels are provided. (b) UMAP plots colored by G.T dihedral conformations of RECOVAR and DRGN-AI at different noise levels. Higher noise demonstrates thicker representations.
%     \label{fig:fig7_noise}
%   \end{minipage}%
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%     More space
%     %\input{Tables/004_table}
%   \end{minipage}
% \end{figure}










% \begin{figure}[h]
%   \centering
%   \begin{minipage}[t]{0.45\textwidth}
%     % \centering
%     \includegraphics[width=\textwidth]{Figures/pngs/Fig7_noise.pdf}
%     \caption{\textbf{IgG-1D Noise.}} (a) AUC of Per-Conformation-FSC for each method at SNR levels of 0.01, 0.005, 0.001, respectively. cryo-EM images at different noise levels are provided. (b) UMAP plots colored by G.T dihedral conformations of RECOVAR and DRGN-AI at different noise levels. Higher noise demonstrates thicker representations.
%     \label{fig:fig7_noise}
%   \end{minipage}\hfill
%   \begin{minipage}[h]{0.45\textwidth}
%   % \captionsetup{type=table, justification=raggedright, singlelinecheck=false} % Left-align table caption
%     \centering
%     % \captionsetup{type=table} % Change the type to table for correct numbering
%     % \addtocounter{table}{1} % Manually adjust the table counter
%     \begin{tabular}[H]{c|c|c}
%         % \centering
%         \toprule
%         \textbf{Method} &
%         \textbf{Ribosembly} & \textbf{Tomotwin-100} \\
%        % & k= & k=5\%  \\
%         \midrule
%         CryoDRGN &  78.84 (0.14) & \textbf{96.78 (0.13)}\\
        
%         DrgnAI-fixed & 76.62 (0.16) & 85.55 (0.08)  \\
        
%         Opus-DSD & 72.53 (0.46) & 50.30 (0.17) \\
        
%         3DVA & 72.05 (0.15) & 11.80 (0.05)  \\
        
%         RECOVAR & \textbf{78.89 (0.06)}& 39.89 (0.19)\\
%         \midrule

%         CryoDRGN2 &  53.37 (0.12)& \textbf{15.01 (0.07)}\\
%         DrgnAI-abinit & \textbf{66.27 (0.14)}& 11.13 (0.14)\\
%         \bottomrule
%       \end{tabular}
%     \captionof{table}{\textbf{Ribosembly and Tomotwin-100 percentage of correct structural clustering.} Percentage of matching neighbors (Eq. \ref{eq:neigh_sim}) with $k$ equal to the number of ground truth images per structure. The mean from five independent subsets is presented, and standard deviation of the mean is shown in parenthesis.}
%     \label{tab:tab2_cluster}
%   \end{minipage}
% \end{figure}





% \begin{figure}[h]
%   \centering
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/pngs/Fig7_noise.pdf}
%     \caption{IgG-1D Noise.} (a) AUC of Per-Conformation-FSC for each method at SNR levels of 0.01, 0.005, 0.001, respectively. cryo-EM images at different noise levels are provided. (b) UMAP plots colored by G.T dihedral conformations of RECOVAR and DRGN-AI at different noise levels. Higher noise demonstrates thicker representations.
%     \label{fig:fig7_noise}
%   \end{minipage}%
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%     More space
%     %\input{Tables/004_table}
%   \end{minipage}
% \end{figure}


==> Tables/002_table2.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \resizebox{1\textwidth}{!}{
      \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \toprule
        
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{|c|}{\textbf{Ribosembly}} & \multicolumn{4}{c}{\textbf{Tomotwin-100}} \\
        \cmidrule(r){2-9}
        & \multicolumn{2}{|c|}{No Mask} & \multicolumn{2}{c}{Mask} & \multicolumn{2}{|c|}{No Mask} & \multicolumn{2}{c}{Mask} \\
        % \cmidrule(r){2-9}
        & Mean (std) & Median & Mean (std) & Median & Mean (std) & Median & Mean (std) & Median \\
        \midrule
        CryoDRGN & 0.358 (0.022) & 0.365 & 0.363 (0.022) & 0.37 & \textbf{0.318 (0.034)} & 0.319 & \textbf{0.321 (0.034)} & 0.322 \\
        DRGN-AI-fixed & 0.317 (0.031) & 0.327 & 0.334 (0.032) & 0.344 & 0.193 (0.042) & 0.204 & 0.206 (0.041) & 0.212 \\
        Opus-DSD & 0.214 (0.023) & 0.224 & 0.214 (0.023) & 0.224 & 0.199 (0.034) & 0.206 & 0.199 (0.034) & 0.206  \\
        3DVA & 0.335 (0.021) & 0.341 & 0.341 (0.023) & 0.348 & 0.093 (0.04) & 0.082 & 0.095 (0.04) & 0.083 \\
        RECOVAR & \textbf{0.399 (0.017)} & \textbf{0.405} & \textbf{0.4 (0.017)} & \textbf{0.405} & 0.305 (0.093) & \textbf{0.329} & 0.306 (0.093) & \textbf{0.33} \\
        3D Class & 0.215 (0.061) & 0.217 & 0.233 (0.068) & 0.237 & 0.045 (0.024) & 0.037 & 0.046 (0.026) & 0.037 \\
        \midrule

        CryoDRGN2 & \textbf{0.312 (0.028)} & \textbf{0.326} & \textbf{0.316 (0.029)} & \textbf{0.33} & \textbf{0.076 (0.016)} & \textbf{0.075} & \textbf{0.076 (0.016)} & \textbf{0.074} \\
        DRGN-AI & 0.27 (0.116) & 0.318 & 0.274 (0.118) & 0.324 & 0.073 (0.014) & 0.073 & 0.073 (0.014) & 0.073 \\
        3D Class abinit & 0.099 (0.063) & 0.065 & 0.099 (0.064) & 0.065 & 0.032 (0.012) & 0.031 & 0.032 (0.012) & 0.032 \\
        \bottomrule
      \end{tabular}
    }
    \caption{\textbf{AUC of Per-Conformation-FSC on Ribosembly and Tomotwin-100.}}
    \label{tab:tab2_assemble_mix}
\end{table*}


% \begin{table*}[t]
%   \centering
%   \footnotesize
%   \resizebox{1\textwidth}{!}{
%       \begin{tabular}{c|c|c|c|c|c|c|c|c}
%         \toprule
        
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{|c|}{\textbf{Assemble-het}} & \multicolumn{4}{c}{\textbf{Mix-het}} \\
%         \cmidrule(r){2-9}
%         & \multicolumn{2}{|c|}{No Mask} & \multicolumn{2}{c}{Mask} & \multicolumn{2}{|c|}{No Mask} & \multicolumn{2}{c}{Mask} \\
%         \cmidrule(r){2-9}
%         & Mean (std) & Median & Mean (std) & Median & Mean (std) & Median & Mean (std) & Median \\
%         \midrule
%         CryoDRGN &  &  &  &  &  &  &  &  \\
%         DrgnAI-fixed &  &  &  & & & & & \\
%         Opus-DSD &  &  &  &  & &  &  \\
%         3DVA &  & &  &  &  &  &  &  \\
%         RECOVAR &  &  & & & & &  & \\
%         3D Class &  &  &  & &  & & &  \\
%         \midrule

%         CryoDRGN2 &  & &  & &  & &  &  \\
%         DrgnAI-abinit &  &  &  & &  & &  &  \\
%         3D Class (\textit{ab initio}) &  & &  &  &  & &  & \\
%         \bottomrule
%       \end{tabular}
%     }
%     \caption{\textbf{Quantitative results 1.} \textit{Volume-FSC} is averaged across K-Means centroids (K=20). \textit{End-to-End-FSC} is averaged across 100 reconstructions. Standard deviation is given in parentheses.}
%     \label{tab:tab1_joint}
% \end{table*}



==> Tables/003_table.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \resizebox{1\textwidth}{!}{
      \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Conf-het-1}} & \multicolumn{2}{|c|}{\textbf{Conf-het-2}} & \multicolumn{2}{c}{\textbf{Spike-het}} & \multicolumn{2}{|c|}{\textbf{Mix-het}} & \multicolumn{2}{c}{\textbf{Assemble-het}} \\
        \cmidrule(r){2-11}
        % \cmidrule(r){4-5}
        % \cmidrule(r){6-7}
        % \cmidrule(r){8-9}
        & Volume & End-to-End & Volume & End-to-End & Volume & End-to-End & Volume & End-to-End & Volume & End-to-End \\
        \midrule
        3D Class (\textit{fixed}) & 0.435 (0.004) & 0.424 (0.012) & 0.422 (0.005) & 0.400 (0.019) & 0.288 (0.025) & 0.285 (0.016) & 0.366 (0.096) & 0.380 (0.035) & 0.446 (0.004) & 0.432 (0.014) \\
        3DVA & 0.437 (0.005) & 0.423 (0.005) & 0.420 (0.005) & 0.406 (0.007) & 0.297 (0.017) & 0.299 (0.017) & 0.388 (0.007) & 0.394 (0.011) & 0.447 (0.005) & 0.396 (0.018) \\
        % 3DVA & 0.437 (0.005) & 0.397 (0.022) & 0.420 (0.005) & 0.358 (0.029) & 0.297 (0.017) & 0.388 (0.007) & 0.352 (0.040) & 0.447 (0.004) & 0.396 (0.018) \\
        3DFlex & 0.403 (0.004) & 0.397 (0.004) & 0.383 (0.005) & 0.377 (0.006) & 0.220 (0.009) & 0.207 (0.010) & 0.401 (0.002) & \textbf{0.395 (0.004)} & 0.397 (0.004) & 0.391 (0.004) \\
        CryoDRGN & \textbf{0.451 (0.004)} & \textbf{0.446 (0.007)} & \textbf{0.436 (0.007)} & \textbf{0.437 (0.006)} & \textbf{0.316 (0.013)} & \textbf{0.307 (0.015)} & 0.399 (0.004) & 0.370 (0.019) & \textbf{0.463 (0.002)} & \textbf{0.460 (0.007)} \\
        DrgnAI-fixed & 0.438 (0.004) & 0.435 (0.005) & 0.414 (0.004) & 0.411 (0.006) & 0.261 (0.006) & 0.254 (0.010) & \textbf{0.405 (0.004)} & 0.388 (0.017) & 0.441 (0.003)  & 0.439 (0.004) \\
        Opus-DSD & 0.342 (0.004) & 0.338 (0.007) & 0.321 (0.006) & 0.317 (0.010) & 0.167 (0.021) & 0.169 (0.007) & 0.316 (0.003) & 0.304 (0.010) & 0.192 (0.005) & 0.181 (0.011) \\
        RECOVAR & 0.342 (0.004) & 0.338 (0.007) & 0.321 (0.006) & 0.317 (0.010) & 0.167 (0.021) & 0.169 (0.007) & 0.316 (0.003) & 0.304 (0.010) & 0.192 (0.005) & 0.181 (0.011) \\
        E2GMM & 0.342 (0.004) & 0.338 (0.007) & 0.321 (0.006) & 0.317 (0.010) & 0.167 (0.021) & 0.169 (0.007) & 0.316 (0.003) & 0.304 (0.010) & 0.192 (0.005) & 0.181 (0.011) \\
        Dynamight & 0.342 (0.004) & 0.338 (0.007) & 0.321 (0.006) & 0.317 (0.010) & 0.167 (0.021) & 0.169 (0.007) & 0.316 (0.003) & 0.304 (0.010) & 0.192 (0.005) & 0.181 (0.011) \\
        
        \midrule

        3D Class (\textit{ab initio}) & 0.171 (0.068) & 0.183 (0.062) & 0.173 (0.076) & 0.181 (0.065) & 0.209 (0.086) & \textbf{0.251 (0.035)} & 0.133 (0.073) & 0.177 (0.063) & 0.187 (0.071) & 0.192 (0.069) \\
        CryoDRGN2 & 0.368 (0.091) & 0.379 (0.066) & 0.316 (0.038) & 0.312 (0.057) & 0.157 (0.071) & 0.207 (0.052) & 0.355 (0.049) & 0.343 (0.059) & 0.387 (0.008) & 0.404 (0.052) \\
        DrgnAI-abinit & \textbf{0.428 (0.004)} & \textbf{0.420 (0.034)} & \textbf{0.407 (0.002)} & \textbf{0.411 (0.032))} & \textbf{0.257 (0.006)} & 0.250 (0.010) & \textbf{0.389 (0.009)} & \textbf{0.357 (0.051)} & \textbf{0.431 (0.003)} & \textbf{0.424 (0.035)} \\
        % DrgnAI-abinit & \textbf{0.418 (0.005)} & \textbf{0.413 (0.009)} & 0.113 (0.006) & 0.106 (0.008) &  & 0.119 (0.008) & 0.114 (0.008) & 0.121 (0.007) & 0.114 (0.008) \\
        \bottomrule
      \end{tabular}
    }
    % \caption{\textbf{Quantitative results.} \textbf{Conf-het, Comp-het:} \textit{Volume-FSC} and \textit{End-to-End-FSC} metrics at SNR 0.1, with K=10 for Conf-het and Comp-het, \textbf{MD:}\textit{Volume} metric at SNR 0.1, K=10 for MD, \textbf{Conf-het noisy:} \textit{Volume} and \textit{End-to-End} metrics at SNR 0.01, K=10 for Conf-het, \textbf{Conf-het big:} \textit{Volume} and \textit{End-to-End-FSC} metrics at SNR 0.1, K=10 for Conf-het with 10,000 images. Each value represents the mean and standard deviation of \textit{Volume-FSC} and \textit{End-to-End-FSC} AUC \textit{K}-means (K=10).}
    \caption{\textbf{Quantitative results 1.} \textit{Volume-FSC} is averaged across K-Means centroids (K=20). \textit{End-to-End-FSC} is averaged across 100 reconstructions. Standard deviation is given in parentheses.}
    \label{tab:tab1_joint}
\end{table*}


